AMLSI: A Novel Accurate Action Model Learning Algorithm

This paper presents new approach based on grammar induction called AMLSI Action Model Learning with State machine Interactions. The AMLSI approach does not require a training dataset of plan traces to work. AMLSI proceeds by trial and error: it queries the system to learn with randomly generated action sequences, and it observes the state transitions of the system, then AMLSI returns a PDDL domain corresponding to the system. A key issue for domain learning is the ability to plan with the learned domains. It often happens that a small learning error leads to a domain that is unusable for planning. Unlike other algorithms, we show that AMLSI is able to lift this lock by learning domains from partial and noisy observations with sufficient accuracy to allow planners to solve new problems.

==> parts/ablation.tex <==
\begin{table*}[!t]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c||c|c|c|c|c||c|c|c|c|c||c|c|c|c|c||c|c|c|c|c|}
\hline
\multicolumn{2}{|c||}{Fluents} & \multicolumn{10}{|c||}{$100\%$} & \multicolumn{10}{|c|}{$25\%$}\\ \hline
\multicolumn{2}{|c||}{Noise} & \multicolumn{5}{|c||}{$0\%$} & \multicolumn{5}{|c||}{$20\%$} & \multicolumn{5}{|c||}{$0\%$} & \multicolumn{5}{|c|}{$20\%$}\\ \hline
Domain & Algorithm & $E_\rho$ & $E_\epsilon$ & $E_\sigma$ & $Solved$ & $Acc$ & $E_\rho$ & $E_\epsilon$ & $E_\sigma$ & $Solved$ & $Acc$ & $E_\rho$ & $E_\epsilon$ & $E_\sigma$ & $Solved$ & $Acc$ & $E_\rho$ & $E_\epsilon$ & $E_\sigma$ & $Solved$ & $Acc$ \\ \hline\hline
\multirow{4}{*}{Blocksworld}
& AMLSI  & $0$ & $0$ & $0$ & $100$ & $100$
         & $0.8$ & $0.8$ & $0.6$ & $93.7$ & $93.7$
         & $0$ & $0$ & $0$ & $100$ & $100$
         & $2.1$ & $1.5$ & $1.2$ & $76.3$ & $76.3$ \\
& Generation step
         & $0$ & $0$ & $0$ & $100$ & $100$
         & $0$ & $0$ & $33.25$ & $0$ & $0$
         & $0$ & $0$ & $19.1$ & $0$ & $0$
         & $0$ & $0$ & $35.8$ & $0$ & $0$\\
& Simple refinement
         & $0$ & $0$ & $0$ & $100$ & $100$
         & $7.7$ & $6.6$ & $26.3$ & $20$ & $0$
         & $0$ & $0$ & $0$ & $100$ & $100$
         & $0$ & $0$ & $28.7$ & $20$ & $0$\\
& Tabu search alone
         & $0$ & $0$ & $9.8$ & $86.7$ & $13$
         & $0.3$ & $0.5$ & $9.6$ & $87$ & $13$
         & $2.34$ & $4.5$ & $12.3$ & $61.7$ & $9$
         & $2.4$ & $4.7$ & $13.3$ & $67$ & $10.3$\\ \hline \hline
% \multirow{4}{*}{Gripper}
% & AMLSI  & $0$ & $0$ & $0$ & $100$ & $100$
%          & $0$ & $0$ & $0$ & $100$ & $100$
%          & $0$ & $0$ & $0$ & $100$ & $100$
%          & $0$ & $0$ & $0$ & $100$ & $100$ \\
% & Generation step
%          & $0$ & $0$ & $0$ & $100$ & $100$
%          & $0$ & $0$ & $46.9$ & $0$ & $0$
%          & $0$ & $0$ & $0.9$ & $86.7$ & $86.7$
%          & $0$ & $0$ & $37.6$ & $0.7$ & $0$\\
% & Simple refinement
%          & $0$ & $0$ & $0$ & $100$ & $100$
%          & $0$ & $0$ & $46.9$ & $0$ & $0$
%          & $0$ & $0$ & $0$ & $100$ & $100$
%          & $0$ & $0$ & $28.5$ & $13.3$ & $0$\\
% & Tabu search alone
%          & $0$ & $0$ & $0$ & $100$ & $100$
%          & $0$ & $0$ & $0$ & $100$ & $100$
%          & $0$ & $0$ & $0$ & $100$ & $100$
%          & $0$ & $0$ & $0$ & $100$ & $100$ \\ \hline \hline
\multirow{4}{*}{Hanoi}
& AMLSI  & $0$ & $0$ & $0.9$ & $100$ & $100$
         & $0$ & $0$ & $0.9$ & $100$ & $100$
         & $0$ & $0$ & $0.9$ & $100$ & $100$
         & ${0.5}$ & ${0.9}$ & ${2}$ & $93$ & $86.7$ \\
& Generation step
         & $0$ & $0$ & $0.9$ & $100$ & $100$
         & $0$ & $0$ & $37.8$ & $4.3$ & $0$
         & $0$ & $0$ & $23.6$ & $0$ & $0$
         & $0$ & $0$ & $38$ & $4.3$ & $0$\\
& Simple refinement
         & $0$ & $0$ & $0.9$ & $100$ & $100$
         & $0$ & $0$ & $34.8$ & $5$ & $0$
         & $0$ & $0$ & $0.9$ & $100$ & $100$
         & $3.4$ & $0$ & $35$ & $0.7$ & $0$\\
& Tabu search alone
         & $0.8$ & $0$ & $12.7$ & $76.7$ & $0$
         & $0$ & $0$ & $12.8$ & $71.33$ & $0$
         & $3.7$ & $6.6$ & $18.8$ & $53.3$ & $6.7$
         & $4.3$ & $6$ & $19.7$ & $49.3$ & $6.7$\\ \hline \hline
\multirow{4}{*}{N-Puzzle}
& AMLSI
         & $0$ & $0$ & $5.6$ & $100$ & $100$
         & $0$ & $0$ & $5.6$ & $100$ & $100$
         & $0$ & $0$ & $5.6$ & $100$ & $100$
         & $0$ & $0$ & $5.6$ & $100$ & $100$ \\
& Generation step
         & $0$ & $0$ & $5.6$ & $100$ & $100$
         & $0$ & $0$ & $37.4$ & $13.3$ & $0$
         & $0$ & $0$ & $27$ & $1.3$ & $0$
         & $0$ & $0$ & $38.9$ & $0$ & $0$\\
& Simple refinement
         & $0$ & $0$ & $5.6$ & $100$ & $100$
         & $0$ & $0$ & $36$ & $26.7$ & $1.33$
         & $0$ & $0$ & $5.6$ & $100$ & $100$
         & $0$ & $0$ & $38.9$ & $0$ & $0$\\
& Tabu search alone
         & $0$ & $0$ & $5.6$ & $100$ & $100$
         & $0$ & $0$ & $5.6$ & $100$ & $100$
         & $0$ & $0$ & $5.6$ & $100$ & $100$
         & $0$ & $0$ & $5.6$ & $100$ & $100$\\ \hline \hline
\multirow{4}{*}{Peg Solitaire}
& AMLSI  & ${0}$ & $0$ & ${6.7}$ & $100$ & $100$
         & ${3}$ & ${0}$ & $12.3$ & $66.7$ & $66.7$
         & ${0}$ & $0$ & ${7.3}$ & $100$ & $100$
         & ${4}$ & ${0.8}$ & $14$ & ${80}$ & $76.7$ \\
& Generation step
         & ${0}$ & $0$ & $4$ & $0$ & $0$
         & ${0}$ & $0$ & $30.2$ & $0$ & $0$
         & ${0}$ & $0$ & $21.2$ & $0$ & $0$
         & ${0}$ & $0$ & $30.1$ & $0$ & $0$\\
& Simple refinement
         & ${0}$ & $0$ & $4.2$ & $0$ & $0$
         & ${0}$ & $1$ & $30.2$ & $0$ & $0$
         & ${0}$ & $0$ & $4.2$ & $100$ & $0$
         & ${0}$ & $1$ & $30.1$ & $0$ & $0$\\
& Tabu search alone
         & ${0}$ & $0$ & $8.2$ & $0$ & $0$
         & ${0}$ & $0$ & $8.1$ & $0$ & $0$
         & ${0}$ & $0$ & $8.4$ & $20$ & $20$
         & ${0}$ & $0$ & $8.3$ & $20$ & $20$\\ \hline \hline
\multirow{4}{*}{Parking}
& AMLSI  & $0$ & $0$ & $3.9$ & $-$ & -
         & $0$ & $0$ & $3.9$ & $-$ & -
         & $0$ & $0$ & $4.1$ & $-$ & -
         & $0.2$ & $0$ & $4.3$ & $-$ & - \\
& Generation step
         & $0$ & $0$ & $3.9$ & $-$ & -
         & $0$ & $0$ & $30.2$ & $-$ & -
         & $0$ & $0$ & $21.2$ & $-$ & -
         & $0$ & $0$ & $30.9$ & $-$ & -\\
& Simple refinement
         & $0$ & $1$ & $4.2$ & $-$ & -
         & $0$ & $0$ & $30.1$ & $-$ & -
         & $0$ & $1$ & $4.2$ & $-$ & -
         & $0$ & $0$ & $30.7$ & $-$ & -\\
& Tabu search alone
         & $0$ & $0$ & $8.2$ & $-$ & -
         & $0$ & $0$ & $8.1$ & $-$ & -
         & $0$ & $0$ & $8.4$ & $-$ & -
         & $0$ & $0$ & $8.3$ & $-$ & -\\ \hline \hline
\multirow{4}{*}{Zenotravel}
& AMLSI  & $0$ & $0$ & $0$ & $100$ & $100$
         & $0.1$ & $0$ & ${0.2}$ & ${100}$ & $99.3$
         & $0$ & $0$ & $0$ & $100$ & $100$
         & ${0}$ & ${0}$ & ${0}$ & ${100}$ & $100$ \\
& Generation step
         & ${0}$ & $0$ & $0$ & $100$ & $100$
         & $0$ & $0$ & $27.4$ & $14.7$ & $0$
         & $0$ & $0$ & $10$ & $12.6$ & $0$
         & $1.7$ & $3$ & $25.9$ & $19.3$ & $0$\\
& Simple refinement
         & ${0}$ & $0$ & $0$ & $100$ & $100$
         & $0.3$ & $1.9$ & $22.4$ & $21.3$ & $0$
         & ${0}$ & $0$ & $1$ & $92.7$ & $65.6$
         & $2.5$ & $2.4$ & $206$ & $51.3$ & $0$\\
& Tabu search alone
         & ${0}$ & $0$ & $1.8$ & $100$ & $73.3$
         & ${0}$ & $0$ & $5.4$ & $100$ & $33.3$
         & ${0}$ & $0$ & $4.2$ & $100$ & $40$
         & ${0}$ & $0$ & $8.8$ & $100$ & $20$\\ \hline \hline
\end{tabular}
}
\caption{\label{tab:ablation} Ablation study on 5 IPC domains. Performance is measured in terms of error rates for preconditions (resp. effects) $E_\rho$ (resp. $E_\epsilon$), syntactical error $E_{\sigma}$, the rate of solved problem $Solved$ and accuracy $Acc$. We report the averages computed over $15$ runs ($5$ runs over $3$ different initial states).}
\end{center}
\end{table*}


==> parts/std.tex <==
\begin{table}[!t]
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c||c|c|c|c|c|}
\hline
Domain & $E_\rho (\%)$ & $E_\epsilon (\%)$ & $E_\sigma (\%)$ & $Solved (\%)$ & $Acc (\%)$ \\ \hline\hline
Blocksworld   & $0.6$ & $1.2$ & $0.5$ & $7.4$ & $7.4$\\ \hline
Gripper       & $0$ & $0$ & $0$ & $0$ & $0$ \\ \hline
Hanoi         & $0.3$ & $0.7$ & $1$ & $9.2$ & $9.4$ \\ \hline
N-Puzzle      & $0$ & $0$ & $0$ & $0$ & $0$ \\ \hline
Peg Solitaire & $0.2$ & $1.2$ & $1.2$ & $22.7$ & $24.1$\\ \hline
Parking       & $0.3$ & $0$ & $0.4$ & $1.4$ & $1.4$\\ \hline
Zenotravel    & $0$ & $0$ & $0$ & $0$ & $0$\\ \hline
Sokoban       & $0$ & $0$ & $0.5$ & $0.5$ & $9.4$\\  \hline
Neg Visit All & $0$ & $0$ & $0$ & $0$ & $0$ \\ \hline
Neg Elevator  & $0$ & $0$ & $0$ & $0$ & $0$  \\ \hline
\end{tabular}}
\caption{\label{tab:std}Standard deviation between initial states for all domains and metrics for the fourth experimental scenario}
\end{center}
\end{table}


==> parts/with_without_pc.tex <==
\begin{table*}[!t]
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c||c|c|c|c|c||c|c|c|c|c||c|c|c|c|c||c|c|c|c|c|}
\hline
\multicolumn{2}{|c||}{Fluents} & \multicolumn{10}{|c||}{$100\%$} & \multicolumn{10}{|c|}{$25\%$}\\ \hline
\multicolumn{2}{|c||}{Noise} & \multicolumn{5}{|c||}{$0\%$} & \multicolumn{5}{|c||}{$20\%$} & \multicolumn{5}{|c||}{$0\%$} & \multicolumn{5}{|c|}{$20\%$}\\ \hline
Domain & Pairewise constraints & $E_\rho$ & $E_\epsilon$ & $E_\sigma$ & $Solved$ & $Acc$ & $E_\rho$ & $E_\epsilon$ & $E_\sigma$ & $Solved$ & $Acc$ & $E_\rho$ & $E_\epsilon$ & $E_\sigma$ & $Solved$ & $Acc$ & $E_\rho$ & $E_\epsilon$ & $E_\sigma$ & $Solved$ & $Acc$ \\ \hline\hline
\multirow{2}{*}{Blocksworld}
& With   & $0$ & $0$ & $0$ & $100$ & $100$
         & $0.8$ & $0.8$ & $0.6$ & $93.7$ & $93.7$
         & $0$ & $0$ & $0$ & $100$ & $100$
         & $2.1$ & $1.5$ & $1.2$ & $76.3$ & $76.3$ \\
& Without & $19.5$ & $29.1$ & $22.4$ & $-$ & -
          & $12.3$ & $21.3$ & $18.5$ & $-$ & -
          & $19.2$ & $29.8$ & $22.1$ & $-$ & -
          & $13.3$ & $21.8$ & $16.7$ & $-$ & -\\ \hline \hline
\multirow{2}{*}{Gripper}
& With  & $0$ & $0$ & $0$ & $100$ & $100$
         & $0$ & $0$ & $0$ & $100$ & $100$
         & $0$ & $0$ & $0$ & $100$ & $100$
         & $0$ & $0$ & $0$ & $100$ & $100$ \\
& Without & $0$ & $0$ & $0$ & $-$ & -
         & $0$ & $0$ & $0$ & $-$ & -
         & $0$ & $0$ & $0$ & $-$ & -
         & $0$ & $0$ & $0$ & $-$ & -\\ \hline \hline
\multirow{2}{*}{Hanoi}
& With  & $0$ & $0$ & $0.9$ & $100$ & $100$
         & $0$ & $0$ & $0.9$ & $100$ & $100$
         & $0$ & $0$ & $0.9$ & $100$ & $100$
         & ${0.5}$ & ${0.9}$ & ${2}$ & $93$ & $86.7$ \\
& Without & $15.6$ & $30.1$ & $21.8$ & $-$ & -
         & $0$ & $7.1$ & $14.5$ & $-$ & -
         & $15.6$ & $30.1$ & $21.7$ & $-$ & -
         & $3.4$ & $7$ & $14$ & $-$ & -\\ \hline \hline
         \multirow{2}{*}{N-Puzzle}
& With  & $0$ & $0$ & $5.6$ & $100$ & -
         & $0$ & $0$ & $5.6$ & $100$ & -
         & $0$ & $0$ & $5.6$ & $100$ & -
         & $0$ & $0$ & $5.6$ & $100$ & - \\
& Without & $1.1$ & $1.7$ & $6.7$ & $-$ & -
         & $0$ & $0$ & $5.6$ & $-$ & -
         & $1.1$ & $1.7$ & $6.7$ & $-$ & -
         & $0$ & $0$ & $5.6$ & $-$ & -\\ \hline \hline
\multirow{2}{*}{Peg Solitaire}
& With  & ${0}$ & $0$ & ${6.7}$ & $100$ & $100$
         & ${3}$ & ${0}$ & $12.3$ & $66.7$ & $66.7$
         & ${0}$ & $0$ & ${7.3}$ & $100$ & $100$
         & ${4}$ & ${0.8}$ & $14$ & ${80}$ & $76.7$ \\
& Without & $14$ & $28$ & $18.2$ & $-$ & -
         & $4.2$ & $9.2$ & $15.7$ & $-$ & -
         & $8.8$ & $18.8$ & $18.1$ & $-$ & -
         & $7.1$ & $8.6$ & $16.9$ & $-$ & -\\ \hline \hline
\multirow{2}{*}{Zenotravel}
& With  & $0$ & $0$ & $0$ & $100$ & $100$
         & $0.1$ & $0$ & ${0.2}$ & ${100}$ & $99.3$
         & $0$ & $0$ & $0$ & $100$ & $100$
         & ${0}$ & ${0}$ & ${0}$ & ${100}$ & $100$ \\
& Without & $5$ & $14.5$ & $9.6$ & $-$ & -
         & $2.1$ & $9.4$ & $8.4$ & $-$ & -
         & $4.9$ & $13.5$ & $9.4$ & $-$ & -
         & $2.8$ & $8.9$ & $7.5$ & $-$ & -\\ \hline \hline
\end{tabular}
}
\caption{\label{tab:pairewise} Domain learning with and without pairewise constraints during the grammar induction step on 5 IPC domains. Performance is measured in terms of error rates for preconditions (resp. effects) $E_\rho$ (resp. $E_\epsilon$), syntactical error $E_{\sigma}$, the rate of solved problem $Solved$ and accuracy $Acc$. We report the averages computed over $15$ runs ($5$ runs over $3$ different initial states).}
\end{center}
\end{table*}
